A Heat Diffusion Perspective on Geodesic Preserving Dimensionality Reduction

Diffusion-based manifold learning methods have proven useful in representation learning and dimensionality reduction of modern high dimensional, high throughput, noisy datasets. Such datasets are especially present in fields like biology and physics. While it is thought that these methods preserve underlying manifold structure of data by learning a proxy for geodesic distances, no specific theoretical links have been established. Here, we establish such a link via results in Riemannian geometry explicitly connecting heat diffusion to manifold distances. In this process, we also formulate a more general heat kernel based manifold embedding method that we call heat geodesic embeddings. This novel perspective makes clearer the choices available in manifold learning and denoising. Results show that our method outperforms existing state of the art in preserving ground truth manifold distances, and preserving cluster structure in toy datasets. We also showcase our method on single cell RNA-sequencing datasets with both continuum and cluster structure, where our method enables interpolation of withheld timepoints of data. Finally, we show that parameters of our more general method can be configured to give results similar to PHATE (a state-of-the-art diffusion based manifold learning method) as well as SNE (an attraction/repulsion neighborhood based method that forms the basis of t-SNE).

==> tables/clustering_sc.tex <==
\begin{tabular}{lrllll}
\toprule
 data &  Noise level &   Method &                Homogeneity &        Adjusted Rand Score & Adjusted Mutual Info Score  \\
\midrule
Mnist &            0 & Diff-Map &          $0.556 \pm 0.002$ &          $0.347 \pm 0.002$ &          $0.622 \pm 0.002$  \\
Mnist &            0 & Heat-Geo &            $0.785 \pm 0.0$ &            $0.695 \pm 0.0$ &          $0.829 \pm 0.001$  \\
Mnist &            0 &    Phate &           $0.822 \pm 0.01$ &           $0.72 \pm 0.017$ &          $0.835 \pm 0.011$  \\
Mnist &            0 &     TSNE & $\mathbf{0.903 \pm 0.003}$ & $\mathbf{0.871 \pm 0.002}$ & $\mathbf{0.902 \pm 0.003}$  \\
Mnist &            0 &     UMAP &          $0.851 \pm 0.016$ &          $0.846 \pm 0.005$ &           $0.86 \pm 0.015$  \\
\midrule
 Pbmc &            0 & Diff-Map &          $0.026 \pm 0.001$ &            $0.011 \pm 0.0$ &          $0.038 \pm 0.001$  \\
 Pbmc &            0 & Heat-Geo &          $0.734 \pm 0.009$ &          $0.724 \pm 0.019$ &          $0.768 \pm 0.017$  \\
 Pbmc &            0 &    Phate & $\mathbf{0.798 \pm 0.012}$ & $\mathbf{0.818 \pm 0.009}$ &  $\mathbf{0.785 \pm 0.01}$  \\
 Pbmc &            0 &     TSNE &          $0.605 \pm 0.019$ &          $0.437 \pm 0.032$ &          $0.544 \pm 0.022$  \\
 Pbmc &            0 &     UMAP &          $0.177 \pm 0.037$ &          $0.097 \pm 0.033$ &          $0.148 \pm 0.035$  \\
\midrule
\bottomrule
\end{tabular}

==> tables/emb_small.tex <==
\begin{tabular}{lllll}
\toprule
 &  \multicolumn{2}{c}{Swiss roll} & \multicolumn{2}{c}{Tree} \\
 \midrule
       Method &                   Pearson-$\rho$ &                  Spearman-$\rho$ &          Pearson-$\rho$ &                  Spearman-$\rho$  \\
\midrule
    Diffusion Map &          $0.476 \pm 0.226$ &          $0.478 \pm 0.138$ &     $0.538 \pm 0.05$ &          $0.471 \pm 0.089$  \\
       Heat-PHATE &          $0.674 \pm 0.169$ &          $0.684 \pm 0.134$ &     $0.614 \pm 0.02$ &          $0.571 \pm 0.044$ \\
            PHATE &           $0.287 \pm 0.03$ &          $0.349 \pm 0.028$ &     $\mathbf{0.615 \pm 0.017}$ &          $0.572 \pm 0.036$ \\
         Rand-Geo &           $0.39 \pm 0.029$ &           $0.43 \pm 0.022$ &     $0.487 \pm 0.064$ &          $0.465 \pm 0.071$ \\
    Shortest Path &           $0.467 \pm 0.17$ &          $0.511 \pm 0.163$ &     $0.542 \pm 0.047$ &           $0.514 \pm 0.06$ \\
             TSNE &          $0.721 \pm 0.183$ & $\mathbf{0.724 \pm 0.151}$ &      $0.583 \pm 0.042$ &          $0.553 \pm 0.045$ \\
             UMAP & $\mathbf{0.727 \pm 0.181}$ &          $0.713 \pm 0.167$ &     $0.595 \pm 0.032$ &          $0.562 \pm 0.036$ \\
        \methodshort~(ours) &          $0.672 \pm 0.221$ &          $0.676 \pm 0.193$ & $0.613 \pm 0.025$ &  $\mathbf{0.58 \pm 0.036}$ \\
\bottomrule
\end{tabular}

